Fast, Effective, and Self-Supervised: Transforming Masked Language Models into Universal Lexical and Sentence Encoders

Pretrained Masked Language Models (MLMs) have revolutionised NLP in recent years. However, previous work has indicated that off-the-shelf MLMs are not effective as universal lexical or sentence encoders without further task-specific fine-tuning on NLI, sentence similarity, or paraphrasing tasks using annotated task data. In this work, we demonstrate that it is possible to turn MLMs into effective universal lexical and sentence encoders even without any additional data and without any supervision. We propose an extremely simple, fast and effective contrastive learning technique, termed Mirror-BERT, which converts MLMs (e.g., BERT and RoBERTa) into such encoders in 20-30 seconds without any additional external knowledge. Mirror-BERT relies on fully identical or slightly modified string pairs as positive (i.e., synonymous) fine-tuning examples, and aims to maximise their similarity during identity fine-tuning. We report huge gains over off-the-shelf MLMs with Mirror-BERT in both lexical-level and sentence-level tasks, across different domains and different languages. Notably, in the standard sentence semantic similarity (STS) tasks, our self-supervised Mirror-BERT model even matches the performance of the task-tuned Sentence-BERT models from prior work. Finally, we delve deeper into the inner workings of MLMs, and suggest some evidence on why this simple approach can yield effective universal lexical and sentence encoders.

==> backups.tex <==
\begin{table*}[] %[!htbp]
\centering
\begin{tabular}{lcc}
\toprule
model & representation token & Pearson-correlation \\
\midrule
fastText & - & 0.416 \\
GloVe  & - & 0.377 \\
\midrule
sentence-transformers/bert-base-nli-cls-token & [CLS] & 0.648 \\
sentence-transformers/bert-base-nli-stsb-mean-tokens & mean-token & 0.678 \\
bert-base-uncased & [CLS] & 0.037 \\
bert-base-uncased & mean-token & 0.201 \\
roberta-base & [CLS] & -0.007 \\
roberta-base & mean-token & -0.060 \\
\midrule
bert-base-uncased + Sap (google en 10k) & [CLS] & 0.505 \\
bert-base-uncased + Sap (Dutch 10k)& [CLS] & 0.463 \\
bert-base-uncased + Sap (Italian 10k) & [CLS] & 0.462 \\
bert-base-uncased + Sap (random string 10k) & [CLS] & 0.452 \\
bert-base-uncased + Sap (Turkish 10k) & [CLS] & 0.449 \\
bert-base-uncased + Sap (UMLS en 10k) & [CLS] & 0.421 \\
bert-base-uncased + Sap (Quenya 10k) & [CLS] & 0.408 \\
roberta-base + Sap (google en 10k) & [CLS] & 0.175 \\
\bottomrule
\end{tabular}
\caption{Simlex-999.}
\end{table*}


\begin{table*}[] %[!htbp]
\centering
\begin{tabular}{lccc}
\toprule
model & representation token & Pearson-correlation \\
\midrule
fastText & - &  \\
GloVe  & - &  \\
\midrule
sentence-transformers/bert-base-nli-cls-token & [CLS] & 0.607 \\
sentence-transformers/bert-base-nli-stsb-mean-tokens & mean-token & 0.631 \\
bert-base-uncased & [CLS] & 0.104 \\
bert-base-uncased & mean-token & 0.248 \\
bert-base-multilingual-uncased & [CLS] & 0.039 \\
bert-base-multilingual-uncased & mean-token & 0.075 \\
roberta-base & [CLS] & 0.024 \\
roberta-base & mean-token & -0.031 \\
\midrule
bert-base-uncased + Sap (google en 10k) & [CLS] & 0.502 \\
bert-base-uncased + Sap (Dutch 10k)& [CLS] & 0.470 \\
bert-base-uncased + Sap (Italian 10k) & [CLS] & 0.469 \\
bert-base-uncased + Sap (random string 10k) & [CLS] & 0.467 \\
bert-base-uncased + Sap (Turkish 10k) & [CLS] & 0.472 \\
bert-base-uncased + Sap (UMLS en 10k) & [CLS] & 0.451 \\
bert-base-uncased + Sap (Quenya 10k) & [CLS] & 0.444 \\
bert-base-multilingual-uncased + Sap (google en 10k) & [CLS] & 0.240 \\
bert-base-multilingual-uncased + Sap (Turkish 10k) & [CLS] & 0.189 \\
roberta-base + Sap (google en 10k) & [CLS] & 0.175 \\
xlm-roberta-base + Sap (google en 10k) & [CLS] & 0.223 \\
xlm-roberta-base + Sap (Arabic 10k) & [CLS] & 0.191 \\

\bottomrule
\end{tabular}
\caption{Multi-SimLex, English (en).}
\end{table*}

\begin{table*}[] %[!htbp]
\centering
\begin{tabular}{lcc}
\toprule
model & representation token & Pearson-correlation \\
\midrule
fastText & - &  \\
GloVe  & - &  \\
\midrule
asafaya/bert-base-arabic & [CLS] & 0.052 \\
asafaya/bert-base-arabic & mean-token & 0.100 \\
bert-base-multilingual-uncased & [CLS] & 0.029 \\
bert-base-multilingual-uncased & mean-token & 0.094 \\
xlm-roberta-base & [CLS] & 0.005 \\
xlm-roberta-base & mean-token & 0.042 \\
\midrule
asafaya/bert-base-arabic + Sap (Arabic 10k) & [CLS] & 0.356 \\
bert-base-multilingual-uncased + Sap (Arabic 10k) & [CLS] & 0.150 \\
bert-base-multilingual-uncased + Sap (google en 10k) & [CLS] & 0.143 \\
xlm-roberta-base + Sap (Arabic 10k) & [CLS] & 0.189 \\
xlm-roberta-base + Sap (google en 10k) & [CLS] & 0.208 \\
\bottomrule
\end{tabular}
\caption{Multi-SimLex, Arabic (ar).}
\end{table*}


\begin{table*}[] %[!htbp]
\centering
\begin{tabular}{lcc}
\toprule
model & representation token & Pearson-correlation \\
\midrule
fastText & - &  \\
GloVe  & - &  \\
\midrule
tartuNLP/EstBERT & [CLS] & 0.144 \\
tartuNLP/EstBERT & mean-token & 0.102 \\
bert-base-multilingual-uncased & [CLS] & 0.054 \\
bert-base-multilingual-uncased & mean-token & 0.089 \\
xlm-roberta-base & [CLS] & -0.020 \\
xlm-roberta-base & mean-token & -0.014\\
\midrule
tartuNLP/EstBERT + Sap (Estonian 10k) & [CLS] & 0.336 \\
bert-base-multilingual-uncased + Sap (Estonian 10k) & [CLS] & 0.132 \\
bert-base-multilingual-uncased + Sap (google en 10k) & [CLS] & 0.130 \\
xlm-roberta-base + Sap (Estonian 10k) & [CLS] & 0.122 \\
xlm-roberta-base + Sap (google en 10k) & [CLS] & 0.121 \\

\bottomrule
\end{tabular}
\caption{Multi-SimLex, Estonian (et).}
\end{table*}



% word list:
% en: \url{https://raw.githubusercontent.com/first20hours/google-10000-english/master/google-10000-english.txt} \\
% dutch: \url{https://raw.githubusercontent.com/hermitdave/FrequencyWords/master/content/2016/nl/nl_50k.txt}\\
% italian: \url{https://raw.githubusercontent.com/hermitdave/FrequencyWords/master/content/2016/it/it_full.txt} \\
% turkish: \url{https://raw.githubusercontent.com/hermitdave/FrequencyWords/master/content/2016/tr/tr_50k.txt} \\
% quenya: \url{https://eldamo.org/content/word-indexes/words-q.html} \\


\subsubsection{Biomedical Entity Linking}

We randomly select 10k strings from UMLS as the training corpus.

Results: \Cref{tab:bel}.

On scientific datasets, identity-trained SapBERT is quite close to the original SapBERT. On social media, identity-trained SapBERT lags behind more but still not bad, considering there is no training label at all. This makes sense as in scientific datasets, usually strings that look alike belong to the same concept while in the social media, semantics of very different strings might be the same. This is saying that this approach adapts PubMedBERT to a very good surface-form encoders but solving harder synonym relations (e.g. in the social media), does need external knowledge injection.



\begin{table*}[t]
\setlength{\tabcolsep}{3.0pt}
%\renewcommand{\arraystretch}{1.0}
\centering
\small
%\hspace*{-2.7cm}
\centering
\vspace{-2.2em}
\begin{tabular}{lccccccccccccccccccc}
\toprule
& & \multicolumn{11}{c}{scientific language}  & \multicolumn{5}{c}{social media language}\\
\cmidrule[1.0pt]{2-12} \cmidrule[1.0pt]{14-18}
 \multirow{2}{*}{model} & \multicolumn{2}{c}{NCBI} &  &\multicolumn{2}{c}{BC5CDR-d} &  &\multicolumn{2}{c}{BC5CDR-c} & & \multicolumn{2}{c}{MedMentions} & & \multicolumn{2}{c}{AskAPatient} & & \multicolumn{2}{c}{COMETA}   \\
\cmidrule[1.5pt]{2-3}\cmidrule[1.5pt]{5-6}\cmidrule[1.5pt]{8-9}\cmidrule[1.5pt]{11-12}\cmidrule[1.5pt]{14-15}\cmidrule[1.5pt]{17-18}
 & $@1$ & $@5$ & & $@1$ & $@5$ & & $@1$ & $@5$ & & $@1$ & $@5$  & & $@1$ & $@5$ & & $@1$ & $@5$ \\
\cmidrule[1.0pt]{1-20}
\CC{15}\textsc{PubMedBert}& \CC{15}77.8 &\CC{15} 86.9 &\CC{15} &\CC{15} 89.0 &\CC{15} 93.8 &\CC{15} & \CC{15}93.0 &\CC{15} 94.6 &\CC{15} & \CC{15}43.9 & \CC{15}64.7&\CC{15} & \CC{15}42.5 &\CC{15} 49.6 &\CC{15} &\CC{15} 46.8 &\CC{15} 53.2  \\
\CC{15}\ \ \ + \textsc{SapBert} & \CC{15}92.0 & \CC{15}95.6 &\CC{15} & \CC{15}93.5 & \CC{15}96.0 &\CC{15} & \CC{15}96.5 & \CC{15}98.2 & \CC{15} & \CC{15}50.8 & \CC{15}74.4 \CC{15} & \CC{15} & \CC{15}70.5 & \CC{15}88.9 &\CC{15} & \CC{15}65.9&\CC{15}77.9\\
\ \ \ + \textsc{SapBert} (self-dup, 10k, 2 epochs)  & 91.8 & 95.3 && 92.9 & 96.0 && 95.8 & 97.4 && & && & && 59.3 & 73.8 \\
\ \ \ + \textsc{SapBert} (self-dup, 10k, 2 epochs, no dropout) & 86.3 & 89.9 && 91.2 & 94.5 && 94.5 & 96.4 && & && & &&  50.0 & 58.9\\
\ \ \ + \textsc{SapBert} (w/o self-dup\&miner, 10k, 2 epochs) & 85.7 & 90.2\\
\bottomrule
\end{tabular}
\caption{Biomedical Entity Linking (BEL).}
\label{tab:bel}
%\vspace{-2.0em}
\end{table*}


\subsection{Sentence-Level Tasks}




\begin{table*}[] %[!htbp]
\centering
\begin{tabular}{lccc}
\toprule
model & representation token & Pearson & Spearmean \\
\midrule
bert-base-uncased & [CLS] & 0.172 & 0.203 \\
bert-base-uncased & mean-token & 0.469 & 0.464 \\
roberta-base & [CLS] & 0.242 & 0.317 \\
roberta-base & mean-token & 0.092 & 0.129 \\
distilbert-base-uncased & [CLS] & 0.266 & 0.310 \\
distilbert-base-uncased & mean-token & 0.603 & 0.606 \\
distilbert-roberta & [CLS] & 0.242 & 0.254 \\
distilbert-roberta & mean-token & 0.277 & 0.309 \\
sentence-transformers/bert-base-nli-cls-token & [CLS] & 0.736 & 0.762 \\
sentence-transformers/bert-base-nli-cls-token & mean-token & 0.750 & 0.795 \\
sentence-transformers/bert-base-nli-mean-tokens & [CLS] & 0.717 & 0.736 \\
sentence-transformers/bert-base-nli-mean-tokens & mean-token & 0.743 & 0.774 \\
cambridgeltl/SapBERT-from-PubMedBERT-fulltext & [CLS] & 0.776 & 0.762 \\
cambridgeltl/SapBERT-from-PubMedBERT-fulltext & mean-token & 0.774 & 0.763 \\
\midrule
bert-base-uncased + Sap (sts-benchmark train 10k) & [CLS] & 0.677 & 0.658\\
bert-base-uncased + Sap (sts-benchmark train 10k) & mean-token & 0.710 & 0.689 \\
bert-base-uncased + Sap (sts-benchmark train 10k, mean-token) & [CLS] & 0.470 & 0.463 \\
bert-base-uncased + Sap (sts-benchmark train 10k, mean-token) & mean-token & 0.650 & 0.641  \\
roberta-base + Sap (sts-benchmark train 10k) & [CLS] & 0.759 & 0.750 \\
roberta-base + Sap (sts-benchmark train 10k) & mean-token & 0.757 & 0.747  \\
distilbert-base-uncased + Sap (sts-benchmark train 10k) & [CLS] & 0.625 & 0.609\\
distilbert-base-uncased + Sap (sts-benchmark train 10k) & mean-token & 0.644 & 0.624\\
distilrobertae-base-uncased + Sap (sts-benchmark train 10k) & [CLS] & 0.728 & 0.718 \\
distilroberta-base-uncased + Sap (sts-benchmark train 10k) & mean-token & 0.750 & 0.738 \\
\bottomrule
\end{tabular}
\caption{STS benchmark (\url{http://ixa2.si.ehu.eus/stswiki/index.php/STSbenchmark}). $^{\ast}$: copied from \citep{reimers2019sentence}.}
\end{table*}

\begin{table*}[] %[!htbp]
\centering
\begin{tabular}{lccc}
\toprule
model & rep. token & Pearson & Spearmean \\
\midrule
dccuchile/bert-base-spanish-wwm-uncased & [CLS] & 0.509 & 0.449 \\
dccuchile/bert-base-spanish-wwm-uncased & mean-token & 0.595 & 0.514 \\
bert-base-multilingual-uncased & [CLS] & 0.374 & 0.397  \\
bert-base-multilingual-uncased & mean-token & 0.593 & 0.532  \\
\midrule
dccuchile/bert-base-spanish-wwm-uncased + Sap (Spanish sent. 10k) & [CLS] & 0.600 & 0.538 \\
dccuchile/bert-base-spanish-wwm-uncased + Sap (Spanish sent. 10k) & mean-token & 0.634 & 0.556 \\
bert-base-multilingual-uncased + Sap (Spanish sent. 10k) & [CLS] & 0.594 & 0.515 \\
bert-base-multilingual-uncased + Sap (Spanish sent. 10k) & mean-token & 0.631 & 0.538 \\

\bottomrule
\end{tabular}
\caption{Sentence similarity (Spanish) (\url{https://alt.qcri.org/semeval2015/task2/index.php?id=semantic-textual-similarity-for-spanish}).}
\end{table*}



\begin{table*}[] %[!htbp]
\centering
\begin{tabular}{lccc}
\toprule
model & rep. token & Pearson & Spearmean \\
\midrule
rubert-base-cased & [CLS] & 0.149 & 0.470 \\
rubert-base-cased & mean-token & 0.538 & 0.552 \\
bert-base-multilingual-uncased & [CLS] & 0.377 & 0.430  \\
bert-base-multilingual-uncased & mean-token & 0.577 & 0.616  \\
\midrule
rubert-base-cased + Sap (Russian news sent. 10k) & [CLS] & 0.600 & 0.605 \\
rubert-base-cased + Sap (Russian news sent. 10k) & mean-token & 0.628 & 0.635 \\
bert-base-multilingual-uncased + Sap (Russian news sent. 10k) & [CLS] & 0.640 & 0.630 \\
bert-base-multilingual-uncased + Sap (Russian news sent. 10k) & mean-token & 0.700 & 0.697 \\
\bottomrule
\end{tabular}
\caption{Sentence similarity (Russian) (\url{https://github.com/deepmipt/deepPavlovEval}).}
\end{table*}



\begin{table*}[] %[!htbp]
\centering
\begin{tabular}{lccc}
\toprule
model & loss & Pearson & Spearmean \\
\midrule
bert-base-uncased + Sap (sts-benchmark train 10k) & multi-similarity & 0.677 & 0.658\\
bert-base-uncased + Sap (sts-benchmark train 10k) & multi-similarity (w/o mining) & 0.554 & 0.546 \\
bert-base-uncased + Sap (sts-benchmark train 10k) & triplet & 0.441 & 0.434 \\
bert-base-uncased + Sap (sts-benchmark train 10k) & NCA & 0.430 & 0.421 \\
\bottomrule
\end{tabular}
\caption{Ablation study on objective function (using STS benchmark).}
\end{table*}


\begin{table*}[] %[!htbp]
\centering
\begin{tabular}{lcccc}
\toprule
model & augmentation & representation & Pearson & Spearmean \\
\midrule
roberta-base & - & [CLS] & 0.242 & 0.317 \\
roberta-base & - & mean-token & 0.092 & 0.129 \\
\midrule
roberta-base + Sap (sts-benchmark train 10k) & none & [CLS] & 0.732 & 0.721 \\
roberta-base + Sap (sts-benchmark train 10k) & none & mean-token & 0.556 & 0.556 \\
\midrule
roberta-base + Sap (sts-benchmark train 10k) & dropout & [CLS] & 0.759 & 0.750 \\
roberta-base + Sap (sts-benchmark train 10k) & dropout & mean-token & 0.757 & 0.747  \\
\midrule
roberta-base + Sap (sts-benchmark train 10k) & word masking (1) & [CLS] & 0.684 & 0.673 \\
roberta-base + Sap (sts-benchmark train 10k) & word masking (2) & [CLS] & 0.707 & 0.698 \\
roberta-base + Sap (sts-benchmark train 10k) & word masking (3) & [CLS] & 0.717 & 0.708 \\
roberta-base + Sap (sts-benchmark train 10k) & char erase (5) & [CLS] & 0.704 & 0.701 \\
roberta-base + Sap (sts-benchmark train 10k) & char erase (10) & [CLS] & 0.736 & 0.730 \\
roberta-base + Sap (sts-benchmark train 10k) & char erase (15) & [CLS] & 0.711 & 0.709 \\
roberta-base + Sap (sts-benchmark train 10k) & char erase (20) & [CLS] & 0.688 & 0.684 \\
roberta-base + Sap (sts-benchmark train 10k) & comma insertion & [CLS] & 0.659 & 0.646 \\
roberta-base + Sap (sts-benchmark train 10k) & rand char insertion & [CLS] & 0.671 & 0.662 \\
\midrule
roberta-base + Sap (sts-benchmark train 10k) & word masking (1) + dropout & [CLS] & 0.787 & 0.778 \\
roberta-base + Sap (sts-benchmark train 10k) & word masking (2)+ dropout & [CLS] & 0.783 & 0.778 \\
roberta-base + Sap (sts-benchmark train 10k) & word masking (3)+ dropout & [CLS] & 0.717 & 0.709 \\
roberta-base + Sap (sts-benchmark train 10k) & char erase (5) + dropout & [CLS] & 0.793 & 0.788 \\
roberta-base + Sap (sts-benchmark train 10k) & char erase (10) + dropout & [CLS] & \textbf{0.797} & \textbf{0.795} \\
roberta-base + Sap (sts-benchmark train 10k) & char erase (15) + dropout & [CLS] & 0.763 & 0.758 \\
roberta-base + Sap (sts-benchmark train 10k) & char erase (20) + dropout & [CLS] & 0.749 & 0.743 \\
roberta-base + Sap (sts-benchmark train 10k) & comma insertion + dropout & [CLS] & 0.776 & 0.770 \\
roberta-base + Sap (sts-benchmark train 10k) & rand char insertion + dropout & [CLS] & 0.773 & 0.764 \\
\bottomrule
\end{tabular}
\caption{Compare data augmentations (using STS benchmark).}
\end{table*}


% \begin{table*}[t]
% \setlength{\tabcolsep}{3.0pt}
% %\renewcommand{\arraystretch}{1.0}
% \centering
% \small
% %\hspace*{-2.7cm}
% \centering
% \vspace{-2.2em}
% \begin{tabular}{lccccccccccccccccccc}
% \toprule
% & & \multicolumn{11}{c}{scientific language}  & \multicolumn{5}{c}{social media language}\\
% \cmidrule[1.0pt]{2-12} \cmidrule[1.0pt]{14-18}
%  \multirow{2}{*}{model} & \multicolumn{2}{c}{NCBI} &  &\multicolumn{2}{c}{BC5CDR-d} &  &\multicolumn{2}{c}{BC5CDR-c} & & \multicolumn{2}{c}{MedMentions} & & \multicolumn{2}{c}{AskAPatient} & & \multicolumn{2}{c}{COMETA}   \\
% \cmidrule[1.5pt]{2-3}\cmidrule[1.5pt]{5-6}\cmidrule[1.5pt]{8-9}\cmidrule[1.5pt]{11-12}\cmidrule[1.5pt]{14-15}\cmidrule[1.5pt]{17-18}
%  & $@1$ & $@5$ & & $@1$ & $@5$ & & $@1$ & $@5$ & & $@1$ & $@5$  & & $@1$ & $@5$ & & $@1$ & $@5$ \\
% \cmidrule[1.0pt]{1-20}
% \CC{15}\textsc{PubMedBert}& \CC{15}77.8 &\CC{15} 86.9 &\CC{15} &\CC{15} 89.0 &\CC{15} 93.8 &\CC{15} & \CC{15}93.0 &\CC{15} 94.6 &\CC{15} & \CC{15}43.9 & \CC{15}64.7&\CC{15} & \CC{15}42.5 &\CC{15} 49.6 &\CC{15} &\CC{15} 46.8 &\CC{15} 53.2  \\
% \CC{15}\ \ \ + \textsc{SapBert} & \CC{15}92.0 & \CC{15}95.6 &\CC{15} & \CC{15}93.5 & \CC{15}96.0 &\CC{15} & \CC{15}96.5 & \CC{15}98.2 & \CC{15} & \CC{15}50.8 & \CC{15}74.4 \CC{15} & \CC{15} & \CC{15}70.5 & \CC{15}88.9 &\CC{15} & \CC{15}65.9&\CC{15}77.9\\
% \ \ \ + \textsc{SapBert} (10k, head, 5 epochs)  & 89.3 & 93.6 && 93.4 & 95.8 && 96.1 & 97.2 \\
% \ \ \ + \textsc{SapBert} (10k, head, 10 epochs)  & 88.9 & 94.4 && 93.5 & 96.2 && 96.0 & 97.6 \\
% \ \ \ + \textsc{SapBert} (10k, head, iter0+iter1, 10 epochs)  &  89.4 & 94.4 && 94.5 & 96.4 &&  95.8 & 97.8 \\

% \ \ \ + \textsc{SapBert} (10k, tail) & 87.4 & 92.3 && 92.3 & 95.1 && 95.7 & 97.7 \\
% \ \ \ + \textsc{SapBert} (10k, middle) & 88.1 & 91.8 && 92.3 & 95.4 && 95.9 & 97.2  \\
% \ \ \ + \textsc{SapBert} (10k, random) & 88.3 & 92.3 && 92.6 & 95.7  && 95.7 & 97.2\\

% \bottomrule
% \end{tabular}
% \caption{}
% \label{tab:sap_bert_vs_sota}%}
% \vspace{-2.0em}
% \end{table*}

